CP-mtML: Coupled Projection multi-task Metric Learning for Large Scale Face Retrieval

We propose a novel Coupled Projection multi-task Metric Learning (CP-mtML) method for large scale face retrieval. In contrast to previous works which were limited to low dimensional features and small datasets, the proposed method scales to large datasets with high dimensional face descriptors. It utilises pairwise (dis-)similarity constraints as supervision and hence does not require exhaustive class annotation for every training image. While, traditionally, multi-task learning methods have been validated on same dataset but different tasks, we work on the more challenging setting with heterogeneous datasets and different tasks. We show empirical validation on multiple face image datasets of different facial traits, e.g. identity, age and expression. We use classic Local Binary Pattern (LBP) descriptors along with the recent Deep Convolutional Neural Network (CNN) features. The experiments clearly demonstrate the scalability and improved performance of the proposed method on the tasks of identity and age based face image retrieval compared to competitive existing methods, on the standard datasets and with the presence of a million distractor face images.

==> _ <==
\section{Experiments}
\label{sec:experiments}
We are interested in different facial retrieval tasks. The retrieval tasks includes identity based face retrieval and age based face 
retrieval. But, our method can be easily applied to different types of face retrieval tasks such as attribute based face retrieval, 
expression based face retrieval \etc. Our method is quite useful for the tasks which do not have enough training examples. 

\subsection*{Identity based Face Retrieval}
For an query face image $q_x^i$ with identity $i$, we want to retrieve other images of same identity.  
\subsection*{Age based Face Retrieval}
For an query face image $q_x^{a}$ with age $a$, we want to retrieve other face images bearing same age.

\subsection{Data }
We use following different datasets for our experiment purposes.
%
\vspace{0.5em} \\
\textbf{CASIA Web}
\cite{yi2014learning} consists of 494,414 images from 10,575 identities. We utilise this dataset to compute CNN 
features of faces. We train our model in Alexnet~\cite{krizhevsky2012imagenet}. For the face verification task in LFW, 
our features give approximately 89\% on LFW with euclidean distance. This is around 11\% above the performance of Fisher
Vectors~\cite{Simonyan13}. And, metric learning with 10 times of training training examples (\ie 54,000 of training pairs) 
at dimension of 32 gives 92.9$\pm$1.1\%. This performance is without flipping and hybrid metric learning. At this similar 
setting, Fisher Vectors~\cite{Simonyan13} at 128 dimension gives 91.4\% in LFW. This shows that our features are much 
efficient for task such as Retrieval, where compression of data is crucial. Recently, model of state-of-art CNN features
\footnote{http://www.robots.ox.ac.uk/~vgg/software/vgg\_face/} for face verification has been released publicly, we expect 
that the trends of experiments with our features will be similar to their features.
%
\vspace{0.5em} \\
\textbf{Labeled Faces in the Wild} --
LFW~\cite{huang2007labeled} is a well-known dataset for facial analysis tasks particularly verification and retrieval. 
It consists of more than 13,000 images of with around 5,000 identities. We use this dataset for 
training and testing during identity based face retrieval. We choose one random images from the identities having more than 
5 images as query and rest is used for training purposes similar to~\cite{bhattarai2014some}. We also use identities (dis-)similarity  
pairs as auxiliary tasks while doing age based face retrieval. 
%
\vspace{0.5em} \\
\textbf{MORPH}
MORPH~\cite{ricanek2006morph} is a popular dataset for age estimation. This dataset consists of around 55,000 images annotated 
with both age and identity. There are around 13,000 identities, each having on an average 4 images at different ages. So as to 
prevent identity based pairings, we randomly selected an image from each of the identities and make a subset of dataset for 
our experiments purposes. We use this dataset for both auxiliary task and main task. For auxiliary task, we randomly sample 
1000 images from the this subset of dataset and prepared positive and negative pairs based on the ages. These pairs are 
used to learn the parameters along with main tasks. While as main tasks, we used these pairs for training purposes and selected 
another 2000 images for testing purpose. One randomly selected image from an age category is selected as query and rest are 
set as ground truths. 
%
\vspace{0.5em} \\
\textbf{Expression Dataset}
We use FACES~\cite{ebner2010faces} for expression matching purpose. This dataset contains 2052 images in total from 171 
identities. Each identity has 6 different expressions ( neutrality, happiness, anger, fear, disgust, and sadnes) and 2 images 
for each expressions (171 $\times$ 6 $\times$ 2 = 2052). We choose one randomly selected image of a person from every expressions
This prevents us from making positive identity based pairings. We prepared positive and negative pairs based on the expressions.  
%
%\vspace{0.5em} \\
%\textbf{Attribute Dataset}
%We use celebA~\cite{} dataset for attribute matching purpose. We take a subset of dataset from it for our experiment purpose. 
%We further split this subset into two disjoint sets. One disjoint set will be used for training purpose and another split 
%will be used for retrieval purpose. 
%
\vspace{0.5em} \\
\textbf{Secular Distractors}
There are 1M images extracted from flicker. These are randomly crawled images and these images are  
not biased to any of the task specific datasets. We use these datasets as distractors during retrieval.
%

\subsection{Data Preprocessing and Features}
We perform all the experiments in following sets of features
\vspace{0.5em} \\
\textbf{Local Binary Patterns (LBP)} \\
\textbf{Convolutional Neural Networks (CNN)}

\subsection{Baselines}
We compared proposed methods with following baselines
\vspace{0.5em} \\
\textbf{WPCA}
We compute Whitend
%
\vspace{0.5em} \\
\textbf{Single Task Metric Learning (stML) }
Task specific low dimensional matrix is learnt for each of the task. In the proposed algorithm~\ref{algo:ml}, if we set $\gamma_0 =0$ and 
$L_0$ as zero matrix, we will have stML.
%
\vspace{0.5em} \\
\textbf{Uniform Tasks Metric Learning (utML) }
We learn a projection matrix from union of training examples from main task and auxiliary task. In the proposed algorithm~\ref{algo:ml}, 
if we set $\gamma_0 =0$, $L_0$ as zero matrix, and set $2 \times \texttt{niters}$, we will have utML.
%
\vspace{0.5em} \\
\textbf{mtLMNN }
We use pubicly available code in authors webpage\footnote{http://www.cs.cornell.edu/~kilian/code/code.html}.
%
\subsection{Experiment Results}
We have following sets of retrieval experiments
\vspace{0.5em} \\
\textbf{Parameter Selection}
For choosing parameters while learning projection matrix and to compare our performance with the existing MTML,
we create a sub-set of training pairs. We randomly sample 500 positive and 500 negative pairs from LFW training pairs.
We carefully excluded training pairs in which at least an image is one of the query images. For better compression 
and performance trade-off we choose dimension of 32. We report here the identity retrieval performance  
when auxiliary task is expression matching. We evaluate here separate performance due to $L_0$, $L_t$, and $ L_0+L_t $ 
on identity based face retrieval. In the Table~\ref{table:perf_comoponent_mats}, $L_0, L_1,$ and $L_2$ represent
common, identity specific and expression specific projection matrices.
\begin {table}[h]
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\centering
\footnotesize
\begin{tabular}{ | l | c | c |  c| r |}
\hline                       
Matrix\textbackslash Precision &  @10       &  @20   & @50  & @100  \\
\hline
$L_0$                          &  31.9      & 42.6   &54.4  & 62.4  \\
\hline
$L_1$                          &  34.3      & 40.7   &51.8  & 63.6 \\
\hline
$L_2$                          &  3.5       & 8.7    &15.8  & 24.1 \\
\hline
$L_0+L_1$                      & \bf{ 40.2} & \bf{46.3} & \bf{57.2} & \bf{67.4}  \\
\hline
\end{tabular}
\caption{ Performance of individual matrices in mtML}
\label{table:perf_comoponent_mats}
\end {table}

\begin{figure}[t]
\centering
\includegraphics[width=0.50\textwidth, trim=20 3 25 22, clip]{plots/cv_Aux_Exp_dim_32.pdf} 
\vspace{-0.8em} \\
\caption{
    Retrieval Performance comparison in Cross-Validation Set 
}
\label{fig:graphs}
\end{figure}
%
Following are subtopics of experiments
\vspace{0.5em} \\
\textbf{Main Task: Identity Retrieval, Aux Task: Expression Matching} \\
\textbf{Main Task: Identity Retrieval, Aux Task: Age Matching} \\
\textbf{Main Task: Age Retrieval, Aux Task: Identity Matching}  \\


